SoK: How Robust is Image Classification Deep Neural Network Watermarking? (Extended Version)

Deep Neural Network (DNN) watermarking is a method for provenance verification of DNN models. Watermarking should be robust against watermark removal attacks that derive a surrogate model that evades provenance verification. Many watermarking schemes that claim robustness have been proposed, but their robustness is only validated in isolation against a relatively small set of attacks. There is no systematic, empirical evaluation of these claims against a common, comprehensive set of removal attacks. This uncertainty about a watermarking scheme's robustness causes difficulty to trust their deployment in practice. In this paper, we evaluate whether recently proposed watermarking schemes that claim robustness are robust against a large set of removal attacks. We survey methods from the literature that (i) are known removal attacks, (ii) derive surrogate models but have not been evaluated as removal attacks, and (iii) novel removal attacks. Weight shifting and smooth retraining are novel removal attacks adapted to the DNN watermarking schemes surveyed in this paper. We propose taxonomies for watermarking schemes and removal attacks. Our empirical evaluation includes an ablation study over sets of parameters for each attack and watermarking scheme on the CIFAR-10 and ImageNet datasets. Surprisingly, none of the surveyed watermarking schemes is robust in practice. We find that schemes fail to withstand adaptive attacks and known methods for deriving surrogate models that have not been evaluated as removal attacks. This points to intrinsic flaws in how robustness is currently evaluated. We show that watermarking schemes need to be evaluated against a more extensive set of removal attacks with a more realistic adversary model. Our source code and a complete dataset of evaluation results are publicly available, which allows to independently verify our conclusions.

==> tables/attacks_categories.tex <==
\begin{tabular}{ccccc}
\hline
\textbf{Attack}                           & \textbf{Access} & \textbf{Verifiability} & \textbf{Data Domain} & \textbf{Speed} \\ \hline
\multicolumn{1}{c|}{}                     & \multicolumn{4}{c}{Input Preprocessing}                                        \\
\multicolumn{1}{c|}{All attacks}          & wb                   & bb                     & -      & Fast           \\ \hline
\multicolumn{1}{c|}{}                     & \multicolumn{4}{c}{Model Modification}                                         \\
\multicolumn{1}{c|}{FTLL}          & wb                   & wb                     & Label           & Fast           \\
\multicolumn{1}{c|}{FTAL}          & wb                   & wb                     & Label          & Fast           \\
\multicolumn{1}{c|}{Remainder}            & wb                   & wb                     & Domain         & Fast           \\ \hline
\multicolumn{1}{c|}{}                     & \multicolumn{4}{c}{Model Extraction}                                           \\
\multicolumn{1}{c|}{Retraining}           & bb                   & wb                     & Domain          & Slow           \\
\multicolumn{1}{c|}{Knockoff}             & bb                   & wb                     & Transfer           & Slow           \\
\multicolumn{1}{c|}{Transfer Learning}    & bb                   & wb                     & Domain           & Medium         \\ \hline
\multicolumn{1}{c|}{}                     & \multicolumn{4}{c}{Adapted Model Extraction}                                   \\
\multicolumn{1}{c|}{Adv. Training} & bb                   & wb                     & Domain           & Slow           \\ \hline
\end{tabular}

==> tables/results_mnist.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & Zhang   Content    & Zhang Noise  & Zhang Unrelated & Adi          & Jia          & Li           \\ \hline
Model   Extraction     & 0.101/0.9714       & 0.101/0.9745 & 0.027/0.9740    & 0.100/0.9760 & 0.669/0.9543 & 0.100/0.9829 \\ \hline
Regularization         & 0.106/0.9772       & 0.104/0.9819 & 0.082/0.9801    & 0.113/0.9796 & 0.776/0.9620 & 0.100/0.9886 \\ \hline
Fine Tuning (FTLL)     & 0.994/0.9865       & 1.000/0.9919 & 0.999/0.9839    & 0.897/0.9844 & 0.833/0.9647 & 0.964/0.9894 \\ \hline
Fine Tuning (FTAL)     & 0.754/0.9832       & 0.805/0.9831 & 0.928/0.9806    & 0.749/0.9824 & 0.113/0.9818 & 0.136/0.9815 \\ \hline
Fine Tuning (RTLL)     & 0.703/0.9881       & 0.896/0.9893 & 0.997/0.9896    & 0.563/0.9898 & 0.709/0.9869 & 0.959/0.9882 \\ \hline
Fine Tuning (RTAL)     & 0.169/0.9825       & 0.216/0.9825 & 0.721/0.9888    & 0.418/0.9844 & 0.130/0.9848 & 0.100/0.9793 \\ \hline
Fine Pruning           & 0.101/0.9818       & 0.102/0.9606 & 0.360/0.9728    & 0.100/0.9592 & 0.112/0.9780 & 0.100/0.9767 \\ \hline
Transfer Learning      & 0.101/0.9684       & 0.100/0.9808 & 0.036/0.9681    & 0.103/0.9859 & 0.363/0.9559 & 0.128/0.9832 \\ \hline
Weight Pruning         & 0.999/0.9800       & 1.000/0.9833 & 1.000/0.9809    & 0.752/0.9501 & 0.999/0.9526 & 0.601/0.9457 \\ \hline
Input Reconstruction   & 0.199/0.9825       & 0.122/0.9774 & 0.166/0.9779    & 0.146/0.9821 & 0.887/0.9419 & 0.100/0.9877 \\ \hline
Input Noising          & 0.999/0.9811       & 1.000/0.9833 & 0.998/0.9555    & 0.878/0.9676 & 0.999/0.9473 & 0.949/0.9806 \\ \hline
Input Smoothing        & 0.998/0.9494       & 0.812/0.9748 & 1.000/0.9818    & 0.308/0.9596 & 0.878/0.9442 & 0.134/0.9824 \\ \hline
Input Quantization     & 1.000/0.9917       & 1.000/0.9891 & 0.896/0.9847    & 0.858/0.9857 & 1.000/0.9572 & 0.262/0.9789 \\ \hline
JPEG Compression       & 1.000/0.9814       & 1.000/0.9829 & 1.000/0.9815    & 0.788/0.9883 & 0.979/0.9503 & 0.187/0.9861 \\ \hline
Feature Squeezing      & 1.000/0.9918       & 1.000/0.9891 & 0.890/0.9900    & 0.924/0.9876 & 0.999/0.9509 & 0.986/0.9874 \\ \hline
Knockoff Nets          & 0.983/0.9807       & 0.990/0.8881 & 0.999/0.9017    & 0.510/0.8980 & 0.973/0.8669 & 0.160/0.9493 \\ \hline
Adversarial Training   & 0.958/0.9864       & 0.839/0.9903 & 0.919/0.9918    & 0.593/0.9925 & 0.340/0.9659 & 0.402/0.9886 \\ \hline
Neural Unlearning      & 0.738/0.9896       & 1.000/0.9906 & 0.968/0.9880    & 0.275/0.9858 & 0.131/0.9713 & 0.159/0.9877 \\ \hline
Neural Pruning         & 0.999/0.9833       & 1.000/0.9889 & 1.000/0.9893    & 0.335/0.9668 & 0.960/0.8634 & 0.959/0.9751 \\ \hline
Neural Laundering      & 0.101/0.9714       & 0.100/0.9834 & 0.015/0.9838    & 0.080/0.9845 & 0.095/0.9838 & 0.100/0.9860 \\ \hline
\multicolumn{1}{|l|}{} & Frontier Stitching & Deepmarks    & Blackmarks      & Deepsigns    & Uchida       & Dawn         \\ \hline
Model   Extraction     & 0.640/0.9753       & 0.100/0.9840 & 0.167/0.9847    & 0.130/0.9735 & 0.091/0.9741 & 0.180/0.9741 \\ \hline
Regularization         & 0.760/0.9815       & 0.100/0.9828 & 0.100/0.9811    & 0.308/0.9831 & 0.970/0.9785 & 0.000/0.0000 \\ \hline
Fine Tuning (FTLL)     & 0.694/0.9875       & 1.000/0.9920 & 0.820/0.9895    & 1.000/0.9924 & 1.000/0.9891 & 0.000/0.0000 \\ \hline
Fine Tuning (FTAL)     & 0.646/0.9778       & 0.100/0.9738 & 0.232/0.9802    & 0.688/0.9936 & 1.000/0.9908 & 0.000/0.0000 \\ \hline
Fine Tuning (RTLL)     & 0.724/0.9882       & 1.000/0.9909 & 0.412/0.9896    & 1.000/0.9920 & 1.000/0.9875 & 0.000/0.0000 \\ \hline
Fine Tuning (RTAL)     & 0.670/0.9903       & 0.100/0.9778 & 0.184/0.9801    & 0.550/0.9907 & 1.000/0.9901 & 0.000/0.0000 \\ \hline
Fine Pruning           & 0.580/0.9683       & 0.100/0.9675 & 0.200/0.9742    & 0.520/0.9852 & 1.000/0.9862 & 0.000/0.0000 \\ \hline
Transfer Learning      & 0.586/0.9780       & 0.100/0.9833 & 0.190/0.9686    & 0.190/0.9721 & 0.077/0.9825 & 0.184/0.9683 \\ \hline
Weight Pruning         & 0.604/0.9506       & 0.904/0.9717 & 0.988/0.9664    & 1.000/0.9912 & 1.000/0.9860 & 0.000/0.0000 \\ \hline
Input Reconstruction   & 0.892/0.9742       & 1.000/0.9881 & 0.184/0.9778    & 1.000/0.9897 & 1.000/0.9859 & 0.000/0.0000 \\ \hline
Input Noising          & 0.922/0.9816       & 1.000/0.9895 & 1.000/0.9876    & 1.000/0.9907 & 1.000/0.9867 & 0.000/0.0000 \\ \hline
Input Smoothing        & 0.832/0.9479       & 1.000/0.9893 & 0.712/0.9527    & 1.000/0.9905 & 1.000/0.9866 & 0.000/0.0000 \\ \hline
Input Quantization     & 0.994/0.9863       & 1.000/0.9892 & 0.892/0.9865    & 1.000/0.9906 & 1.000/0.9865 & 0.000/0.0000 \\ \hline
JPEG Compression       & 0.982/0.9844       & 1.000/0.9896 & 1.000/0.9883    & 1.000/0.9908 & 1.000/0.9865 & 0.000/0.0000 \\ \hline
Feature Squeezing      & 0.988/0.9863       & 1.000/0.9894 & 0.208/0.9847    & 1.000/0.9907 & 1.000/0.9864 & 0.000/0.0000 \\ \hline
Knockoff Nets          & 0.916/0.9769       & 0.100/0.9749 & 0.955/0.9616    & 0.310/0.9610 & 0.587/0.9777 & 0.281/0.9819 \\ \hline
Adversarial Training   & 0.874/0.9921       & 0.404/0.9910 & 0.580/0.9905    & 0.481/0.9899 & 1.000/0.9888 & 0.000/0.0000 \\ \hline
Neural Unlearning      & 0.754/0.9897       & 0.364/0.9880 & 0.136/0.9887    & 0.758/0.9923 & 1.000/0.9881 & 0.000/0.0000 \\ \hline
Neural Pruning         & 0.808/0.9492       & 1.000/0.9893 & 0.520/0.9676    & 1.000/0.9898 & 1.000/0.9864 & 0.000/0.0000 \\ \hline
Neural Laundering      & 0.706/0.9878       & 0.100/0.9879 & 0.067/0.9837    & 0.273/0.9903 & 0.190/0.9863 & 0.000/0.0000 \\ \hline
\end{tabular}
